DomainNet: Homograph Detection for Data Lake Disambiguation

Modern data lakes are deeply heterogeneous in the vocabulary that is used to describe data. We study a problem of disambiguation in data lakes: how can we determine if a data value occurring more than once in the lake has different meanings and is therefore a homograph? While word and entity disambiguation have been well studied in computational linguistics, data management and data science, we show that data lakes provide a new opportunity for disambiguation of data values since they represent a massive network of interconnected values. We investigate to what extent this network can be used to disambiguate values. DomainNet uses network-centrality measures on a bipartite graph whose nodes represent values and attributes to determine, without supervision, if a value is a homograph. A thorough experimental evaluation demonstrates that state-of-the-art techniques in domain discovery cannot be re-purposed to compete with our method. Specifically, using a domain discovery method to identify homographs has a precision and a recall of 38% versus 69% with our method on a synthetic benchmark. By applying a network-centrality measure to our graph representation, DomainNet achieves a good separation between homographs and data values with a unique meaning. On a real data lake our top-200 precision is 89%.

==> SECTIONS/structure.tex <==
\section{Structure of repository}

All latex macros, shortcuts, new definitions will be maintained in a separate document called
\verb|datalabmacros.tex|. This allows to share useful latex tricks and favorite macros across documents and projects.

If the papers gets large, it may be better to split up the document and maintain separate sections in the
\verb|SECTIONS/| folder and used with the \verb|\insert| command.
For example, this subsection is inserted with
\verb|\input{SECTIONS/structure}|.
This allows you to comment out some sections while you are working on others, and make it compile faster.

All figures are contained in a separate directory \verb|FIG/|.
Use a consistent naming scheme for the figure and start their names with
\verb|Fig_[rest].pdf|. Git repositories should not check in any compiled PDFs (like \verb|main.pdf|). 
Starting all figure PDF files with \verb|Fig_...| allows to use simple rules in the 
\verb|.gitignore| file.

Use descriptive labels for all referenced content, e.g. 
\verb|\label{sec:intro}| for a section,
\verb|\label{ex:flickr}| for an example,
\verb|\label{fig:Fig_MatrixTextGraphics}| for a figure, or
\verb|\label{eq:2pl}| for an equation.

